Batch-Parallel Euler Tour Trees

The dynamic trees problem is to maintain a forest undergoing edge insertions and deletions while supporting queries for information such as connectivity. There are many existing data structures for this problem, but few of them are capable of exploiting parallelism in the batch-setting, in which large batches of edges are inserted or deleted from the forest at once. In this paper, we demonstrate that the Euler tour tree, an existing sequential dynamic trees data structure, can be parallelized in the batch setting. For a batch of $k$ updates over a forest of $n$ vertices, our parallel Euler tour trees perform $O(k \log (1 + n/k))$ expected work with $O(\log n)$ depth with high probability. Our work bound is asymptotically optimal, and we improve on the depth bound achieved by Acar et al. for the batch-parallel dynamic trees problem. The main building block for parallelizing Euler tour trees is a batch-parallel skip list data structure, which we believe may be of independent interest. Euler tour trees require a sequence data structure capable of joins and splits. Sequentially, balanced binary trees are used, but they are difficult to join or split in parallel. We show that skip lists, on the other hand, support batches of joins or splits of size $k$ over $n$ elements with $O(k \log (1 + n/k))$ work in expectation and $O(\log n)$ depth with high probability. We also achieve the same efficiency bounds for augmented skip lists, which allows us to augment our Euler tour trees to support subtree queries. Our data structures achieve between 67--96x self-relative speedup on 72 cores with hyper-threading on large batch sizes. Our data structures also outperform the fastest existing sequential dynamic trees data structures empirically.

==> inputs/model.tex <==
%\subsection{Model}

\myparagraph{Model}
In the analysis of algorithms we use the following work-depth model,
which is closely related to the PRAM but better models current
machines and programming paradigms that are asynchronous and allow
dynamic forking.
We can simulate the model on the CRCW PRAM equipped with the same
operations with an additional $O(\log^{*} n)$ factor in the depth due to
load-balancing. Furthermore, a PRAM algorithm using $P$ processors and
$T$ time can be simulated in our model with $PT$ work and $T$ depth.

\newcommand{\mpram}{MT-RAM}
\newcommand{\tmpram}{MT2-RAM}
\newcommand{\process}{thread}
\newcommand{\processes}{threads}

\newcommand{\forkins}{\texttt{fork}}
\newcommand{\insend}{\texttt{end}}
\newcommand{\allocateins}{\texttt{allocate}}
\newcommand{\freeins}{\texttt{free}}

The \emph{Multi-Threaded Random-Access Machine
(\mpram{})}~\cite{blelloch2018introduction-draft} consists of a set of
\processes{} that share an unbounded memory.  Each \process{} is basically
equivalent to a Random Access Machine---it works on a program stored
in memory, has a constant number of registers, and has standard RAM
instructions (including an \insend{} to finish the computation).  The
\mpram{} extends the RAM with a \forkins{} instruction that takes a positive
integer $k$ and forks $k$ new child \processes{}.  Each child \process{}
receives a unique integer in the range $[1,\ldots,k]$ in its first
register and otherwise has the identical state as the parent, which
has a $0$ in that register.  They all start by running the next
instruction.  When a \process{} performs a \forkins{}, it is suspended until
all the children terminate (execute an \insend{} instruction).  A
computation starts with a single root \process{} and finishes when that
root \process{} ends.  This model supports what is often referred to as
nested parallelism.  If the root \process{} never does a fork, it is a
standard sequential program.
%% To simplify issues of parallel memory
%% allocation we assume there is an \allocateins{} instruction that takes a
%% positive integer $n$ and allocates a contiguous block of $n$ memory
%% locations, returning a pointer to the block, and a \freeins{}
%% instruction that given a pointer to an allocated block, frees it.

A computation can be viewed as a series-parallel DAG in which each
instruction is a vertex, sequential instructions are composed in
series, and the forked sub\processes{} are composed in parallel. The \defn{work}
of a computation is the number of vertices and the \defn{depth} is the length
of the longest path in the DAG.
%% Two instructions are
%% said to be \defn{concurrent} if they are not reachable from each other
%% in the DAG.  We say two instructions \defn{race} if they are
%% concurrent and one writes to the memory location that the other reads
%% or writes.  Since the outcome of racing instructions can depend on
%% their ordering, we assume the outcome of all instructions in a
%% computation must be consistent with some topological ordering of the
%% DAG.
We augment the model with three atomic instructions that are used
by our algorithms: test-and-set (TS), fetch-and-add (FA), and priority-write
(PW) and discuss our model with these operations as the TS, FA, and PW variants
of the \mpram{}. As is standard with the RAM model, we assume that the memory
locations and registers have at most $O(\log M)$ bits, where $M$ is
the total size of the memory used. More details about the model can be found
in~\cite{blelloch2018introduction-draft}.
%\julian{maybe define test-and-set, fetch-and-add and priority-write}\laxman{Added a section in prelims}
%\julian{talk about how our model is related to CRCW PRAM?}

